AALC: Large Language Model Efficient Reasoning via Adaptive Accuracy-Length Control

Large reasoning models (LRMs) achieve impressive reasoning capabilities by generating lengthy chain-of-thoughts, but this "overthinking" incurs high latency and cost without commensurate accuracy gains. In this work, we introduce AALC, a lightweight, accuracy-aware length reward integrated into reinforcement learning that dynamically balances correctness and brevity during training. By incorporating validation accuracy into the reward and employing a smooth, dynamically scheduled length penalty, AALC delays length penalty until target performance is met. Through extensive experiments across standard and out-of-distribution math benchmarks, we show that our approach reduces response length by over 50% while maintaining or even improving the original accuracy. Furthermore, qualitative analysis reveals that our method curbs redundant reasoning patterns such as excessive subgoal setting and verification, leading to structurally refined outputs rather than naive truncation. We also identify that efficiency gains are accompanied by reduced interpretability: models trained with AALC omit some narrative framing and explanatory context. These findings highlight the potential of reward-based strategies to guide LRMs toward more efficient, generalizable reasoning paths.

==> Tables/error_types.tex <==
\begin{table}[t]
\centering
\small
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc}
\toprule
Error Type                            & Base prompt  & KG1 P. &  KG2 P. \\ \midrule
cannot understand documents & 46.43\% & 50.00\%          & 30.30\%          \\
Incomplete graph / poor graph quality & -       & -                & 15.15\%          \\
needs extra common sense knowledge    & 3.57\%  & 4.17\%           & 6.06\%           \\
over-reasoned                         & 14.29\% & 4.17\%           & -                \\
unanswerable                          & 35.71\% & 41.67\%          & 33.33\%          \\
others                                & -       & -           & 15.15\%          \\ \midrule
Grand Total \#Errors                          & 28      & 24               & 33              \\
\bottomrule
\end{tabular}
}
    \caption{Error made by different approaches on the 2WikiMultiHopQA test examples.}
    \label{tab:error_analysis_2wiki}
\end{table}

==> Tables/qa_results.tex <==
% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{method} & EM             & f1             & precision      & recall         \\ \hline
% w/o kg                       & \textbf{0.450} & \textbf{0.628} & \textbf{0.597} & 0.782          \\ \hline
% w/ predicted kg1             & 0.440          & 0.607          & 0.591          & 0.780          \\ \hline
% w/ predicted kg2             & 0.410          & 0.593          & 0.560          & \textbf{0.821} \\ \hline
% w/ predicted kg2 direct      & 0.360          & 0.540          & 0.514          & 0.780          \\ \hline
% \end{tabular}%
% }
% \caption{HotpotQA w/o Reasoning Chain}
% \label{hotpot_no_cot}
% \end{table}

% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% \multicolumn{1}{|c|}{method} & EM             & f1             & precision      & recall         \\ \hline
% w/o kg                       & 0.550          & 0.716          & 0.729          & 0.830          \\ \hline
% w/ predicted kg1             & 0.560          & 0.714          & \textbf{0.732} & 0.805          \\ \hline
% w/ predicted kg2             & \textbf{0.570} & \textbf{0.728} & 0.731          & \textbf{0.872} \\ \hline
% w/ predicted kg2 direct      & \textbf{0.570} & 0.719          & 0.725          & 0.833          \\ \hline
% \end{tabular}%
% }
% \caption{HotpotQA w/ Reasoning Chain}
% \label{hotpot_cot}
% \end{table}

\begin{table*}[t]
\centering
\small
\begin{tabular}{l|cccc|cccc}
\toprule
& \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} \\ \midrule
Methods                 & \multicolumn{4}{c|}{HotpotQA}   & \multicolumn{4}{c}{2WikiMultiHopQA}  \\ \midrule
Base                  & 0.55 & 0.716 & 0.729 & 0.830  &  0.39 & 0.515 & 0.483     & 0.551 \\
% \textbf{0.45} & \textbf{0.628} & \textbf{0.597} & 0.782 \\
G-Full prompt        & 0.56 & 0.714 & \textbf{0.732} & 0.805 &  0.47 & 0.570 & 0.542     & 0.601 \\
% 0.44 & 0.607 & 0.591 & 0.780 \\
SG-Multi prompt         & 0.57 & \textbf{0.728} & 0.731 & \textbf{0.872} & 0.48 & 0.572 & 0.547     & 0.599 \\
% 0.41 & 0.593 & 0.560 & \textbf{0.821} \\                 
SG-One prompt  & \textbf{0.58} & 0.719 & 0.725 & 0.833 & \textbf{0.49} & \textbf{0.585} & \textbf{0.561}   & \textbf{0.611} \\
% 0.36 & 0.540 & 0.514 & 0.780 \\
\bottomrule
\end{tabular}
\caption{CoT setting results. SG-Multi and SG-One generally outperforms G-Full and the base prompt. This demonstrates the importance of explicitly extract and encoding the semantic relations.}
\vspace{-10pt}
\label{tab:cot_results}
\end{table*}

% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% method                  & EM             & f1             & precision      & recall         \\ \hline
% w/o kg                  & \textbf{0.300} & \textbf{0.453} & \textbf{0.409} & \textbf{0.633} \\ \hline
% w/ predicted kg1        & 0.180          & 0.346          & 0.294          & 0.600          \\ \hline
% w/ predicted kg2        & 0.140          & 0.287          & 0.239          & 0.514          \\ \hline
% w/ predicted kg2 direct & 0.170          & 0.310          & 0.267          & 0.504          \\ \hline
% \end{tabular}%
% }
% \caption{2WikiMultiHopQA w/o Reasoning Chain}
% \label{2wiki_no_cot}
% \end{table}

% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% method                  & EM             & f1             & precision      & recall         \\ \hline
% w/o kg                  & 0.390          & 0.515          & 0.483          & 0.770          \\ \hline
% w/ predicted kg1        & 0.470          & 0.570          & 0.542          & \textbf{0.795} \\ \hline
% w/ predicted kg2        & 0.480          & 0.572          & 0.547          & 0.701          \\ \hline
% w/ predicted kg2 direct & \textbf{0.490} & \textbf{0.585} & \textbf{0.561} & 0.714          \\ \hline
% \end{tabular}%
% }
% \caption{2WikiMultiHopQA w/ Reasoning Chain}
% \label{2wiki_cot}
% \end{table}

% \begin{table}[t]
% % \small
% \centering
% \begin{tabular}{l|cccc|cccc}
% \toprule
% & \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c}{EM} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} \\ \midrule
% Methods   & \multicolumn{4}{c|}{CoT setting~\cite{weichain}} & \multicolumn{4}{c}{Few-shot setting~\cite{brown2020language}}       \\ \midrule
% Base                    & 0.39 & 0.515 & 0.483     & 0.770  & \textbf{0.30}   & \textbf{0.453}  & \textbf{0.409}      & \textbf{0.633} \\
% KG1 Prompt         & 0.47 & 0.570 & 0.542     & \textbf{0.795}  & 0.18  & 0.346  & 0.294      & 0.600 \\
% KG2 Prompt         & 0.48 & 0.572 & 0.547     & 0.701 & 0.14  & 0.287  & 0.239      & 0.514 \\                 
% KG2-D Prompt   & \textbf{0.49} & \textbf{0.585} & \textbf{0.561}   & 0.714  & 0.17  & 0.310  & 0.267      & 0.504 \\
% \bottomrule
% \end{tabular}
% \caption{Few-shot Setting Recall Results.}
% \label{tab:2wiki_cot_new}
% \end{table}

% \begin{table}[t]
% \centering \small
% \begin{tabular}{c|cc}
% \toprule
%             & HotPotQA & 2WikiHop \\ \midrule
% Base Prompt & 0.782    & 0.600    \\
% SG-Full     & 0.780    & 0.633    \\
% SG-Multi    & \textbf{0.821}    & 0.514    \\
% SG-One      & 0.780    & 0.504   \\
% \bottomrule
% \end{tabular}
% \caption{Few-shot Setting Recall Results.}
% \label{tab:fewshot_recall_results}
% \end{table}

\begin{table}[t]
\centering \small
\begin{tabular}{c|cc}
\toprule
            & HotPotQA  \\ \midrule
Base Prompt & 0.782        \\
SG-Full     & 0.780        \\
SG-Multi    & \textbf{0.821}      \\
SG-One      & 0.780      \\
\bottomrule
\end{tabular}
\caption{Few-shot Setting Recall Results on HotpotQA.}
\label{tab:fewshot_recall_results}
\vspace{-10pt}
\end{table}
